An Empirical Comparison of Vocabulary Expansion and Initialization Approaches for Language Models

Language Models (LMs) excel in natural language processing tasks for English but show reduced performance in most other languages. This problem is commonly tackled by continually pre-training and fine-tuning these models for said languages. A significant issue in this process is the limited vocabulary coverage in the original model's tokenizer, leading to inadequate representation of new languages and necessitating an expansion of the tokenizer. The initialization of the embeddings corresponding to new vocabulary items presents a further challenge. Current strategies require cross-lingual embeddings and lack a solid theoretical foundation as well as comparisons with strong baselines. In this paper, we first establish theoretically that initializing within the convex hull of existing embeddings is a good initialization, followed by a novel but simple approach, Constrained Word2Vec (CW2V), which does not require cross-lingual embeddings. Our study evaluates different initialization methods for expanding RoBERTa and LLaMA 2 across four languages and five tasks. The results show that CW2V performs equally well or even better than more advanced techniques. Additionally, simpler approaches like multivariate initialization perform on par with these advanced methods indicating that efficient large-scale multilingual continued pretraining can be achieved even with simpler initialization methods. We release our code publicly (https://github.com/AI4Bharat/VocabAdaptation_LLM/tree/CW2V).

==> table_roberta_initialized.tex <==
% \begin{table*} [!t] 
%     % \setlength{\abovecaptionskip}{0cm}
%     \setlength{\belowcaptionskip}{-0.4cm}
%     \footnotesize
%     \centering
%     \setlength{\tabcolsep}{1.2mm}{}
%     \begin{tabular}{lrrrrrrrrrrrrrrrrrr}
%         \toprule
%         & \multicolumn{6}{c}{XNLI} & \multicolumn{6}{c}{NER} & \multicolumn{6}{c}{QA} \\
%         \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19} 
%         & en & hi & ta & ru & de & avg & en & hi & ta & ru & de & avg & en & hi & ta & ru & de & avg\\
%         % \midrule
%         % XLM-V & 10.1 & \underline{60.3} & 22.9 & 39.3 & \textbf{78.2} & \textbf{67.1} & 17.7 & 61.1 & 28.7 & 53.2 & 65.3 & 59.8 & 45.4 & \textbf{76.6} & 67.0 \\
%         \midrule
%         Constrained Word2Vec &  \textbf{86.0} & 34.2 & 34.4 & 35.2 & 40.2 & 46 & \textbf{82.2} & 16.6 & 13.3 & 13.2 & 43.0 & 33.7 & \textbf{90.7} & 4.2 & 2.1 & 10.3 & 19.2 & 25.3 \\
%         OFA & 85.6 & 37.2 & 37.3 & 36.4 & 40.2 & 47.3 & 81.9 & 21.5 & 8.5 & 13.2 & 43.7 & 33.8 & 90.6 & 10.1 & 1.5 & 10.4 & 26.1 & 27.8 \\
%         Multivariate & 85.7 & 33.9 & 34.5 & 34.5 & 40 & 45.7 & 81.8 & 15.4 & 12.5 & 14 & 42.4 & 33.2 & 90.4 & 6.02 & 1.8 & 8.1 & 22.4 & 25.8  \\
%         Univariate & 85.6 & 36.0 & 34.5 & 36.1 & 39.8 & 46.4 & 82.0 & 17.9 & 12.0 & 12.7 & 45.7 & 34.1 & 90.7 & 6.4 & 1.7 & 9.6 & 23.7 & 26.4 \\
%         Mean & 85.5 & 34.4 & 34.7 & 34.9 & 40.2 & 46.0 & 81.5 & 14.6 & 11.8 & 13.2 & 41.9 & 32.6 & 90.5 & 5.2 & 1.7 & 6.7 & 21.6 & 25.2 \\
%         Random & 85.8 & 34.1 & 34.5 & 35.3 & 40.0 & 45.9 & 81.6 & 16.9 & 10.7 & 13.0 & 43.3 & 33.1 & 90.3 & 6.6 & 1.7 & 7.9 & 22.1 & 25.7 \\
%         % \midrule
%         % RoBERTa-Base & 87.0 & 35.0 & 34.2 & 35.4 & 50.5 & 48.4 & 84.3 & 5.2 & 2.9 & 9.3 & 62.6 & 32.9 \\
        
%        \bottomrule
%     \end{tabular}
%     \caption{Performance of the expanded RoBERTa models initialized with Constrained Word2Vec and baselines on 3 multilingual tasks across 5 languages. Models are fine-tuned on the English training set, and performance is evaluated zero-shot on the test sets of other languages. 
%     \textbf{Bold} (\underline{underlined}): best (second-best) result per controlled group.}
%     \label{initialized_models_roberta}
% \end{table*}

